An empirical study on evaluation metrics of generative adversarial networks

Evaluating generative adversarial networks (GANs) is inherently challenging. In this paper, we revisit several representative sample-based evaluation metrics for GANs, and address the problem of how to evaluate the evaluation metrics. We start with a few necessary conditions for metrics to produce meaningful scores, such as distinguishing real from generated samples, identifying mode dropping and mode collapsing, and detecting overfitting. With a series of carefully designed experiments, we comprehensively investigate existing sample-based metrics and identify their strengths and limitations in practical settings. Based on these results, we observe that kernel Maximum Mean Discrepancy (MMD) and the 1-Nearest-Neighbor (1-NN) two-sample test seem to satisfy most of the desirable properties, provided that the distances between samples are computed in a suitable feature space. Our experiments also unveil interesting properties about the behavior of several popular GAN models, such as whether they are memorizing training samples, and how far they are from learning the target distribution.

==> conclusion.tex <==
%!TEX root=main.tex

\section{Conclusion}
\label{conclusion}
This paper presents a comprehensive study of several model agnostic, sample based evaluation metrics for GANs. We examine whether existing metrics satisfy desirable properties through empirical experiments, specifically 
(1) whether they can discriminate GAN-generated samples from real samples, and are sensitive to mode dropping and mode collapsing; 
(2) robustness to certain transformations, e.g., small translations and rotations that preserves the semantic meaning of images; 
and (3) computational efficiency.  
Our results suggest that the choice of the feature space is crucial.
In the convolutional space of a ResNet pre-trained on ImageNet, both MMD and 1-NN accuracy perform well in terms of discriminability, robustness and efficiency. Wasserstein distance is very sample-inefficient, while the Inception Score seems unsuitable for datasets very different from ImageNet, and is unable to detect overfitting. 
We will release our source code for all these metrics, providing researchers with off-the-shelf tools to compare and improve their GANs.

Based on the two most promising metrics, MMD and 1-NN accuracy, we study the overfitting problem on DCGAN and WGAN. Contrary to the belief by some researchers that GANs memorize the training data, we find that overfitting (at least in the notion we defined) does not occur outside the regime of extremely few training samples. 
This raises an interesting question for the generalization of GANs in contrast to that in supervised learning. 
We hope that future works can contribute to explaining this phenomenon.


==> feature.tex <==
%!TEX root=main.tex
%\vspace{-2 ex}
\section{Feature space}

%\vspace{-2 ex}
%\begin{wrapfigure}{r}{0.41\textwidth}
%      \vspace{-4 ex}
%      \centering
%      \includegraphics[width=0.2\textwidth]{figures/celeba_10nn_shift4_pixel_7x7.png}
%      \includegraphics[width=0.2\textwidth]{figures/celeba_10nn_shift4_conv_7x7.png}\\
%            %\includegraphics[width=0.5\textwidth]{figures/visual_earlyexit_cifar10-2.pdf}
%      \caption{Shifted images (in green box) and their 10 nearest neighbors in the pixel space (\emph{left}) and in the ResNet feature space (\emph{right}).}
%      \vspace{-2 ex}
%      \label{fig:robust_shift}
%\end{wrapfigure}

All of the metrics introduced in the previous section, except for the Inception Score, access the samples $\bx$ through pair-wise distances. The Kernel MMD metric requires a predetermined kernel function $k$, which is typically set to an isotopic Gaussian, while the Wasserstein distance and 1-NN accuracy use the underlying distance metric $d$ directly. The Fr\'echet Inception Distance models the real and generated distributions as multivariate Gaussians in some suitable feature space. All of these methods are highly sensitive to the choice of feature space.

%We consider the class of kernel functions and distances formed by mapping $\bx$ with a fixed feature extractor $\phi$ and computing the usual inner product and Euclidean distance in the resulting feature space.

It is well established that pixel representations of images do not give rise to meaningful Euclidean distances~\citep{forsyth2011computer}. Small translations, rotations, or changes in illumination can incur large distances but typically have little effect on the image content.
To quantity the similarity between distributions of images, it is therefore desirable to use distances that are invariant to such transformations.
The choice of distance function can be re-interpreted as a choice of representation, by defining the distance in a more general form as $d(\bx,\bx')=\|\phi(\bx)-\phi(\bx')\|_2$, where $\phi(\cdot)$ is some general mapping of the input into a semantically meaningful feature space. For Kernel MMD, this corresponds to computing the usual inner product in the feature space $\phi(\mathcal{X})$.

% The choice of this mapping $\phi$ controls the degree to which \emph{the induced distance is sensitive to identity-preserving transformations}.
% Since $\mathbb{P}_r$ is supported over the natural images, we expect $\mathbb{P}_r$ to have certain invariants, e.g. if $\bx, \bx' \in \mathcal{X}$ are the same up to a small translation or a local distortion (small diffeomorphism), we should have $p_r(\bx) \approx p_r(\bx')$ where $p_r$ is the density of $\mathbb{P}_r$. Thus if we apply such transformations to the samples in $S_r$ to produce $S_r'$, we expect that $\hat{\rho}(S_r,S_r') \approx 0$.

%We now consider the invariance properties of different choices of feature spaces. The most straightforward is the raw pixel space $\mathcal{X}$, corresponding to $\phi$ being the identity mapping. As expected, the distance induced by the pixel space is very sensitive. This makes distance-based metric problematic, as also addressed in \citep{theis2015note}. It partly explains why those well-known metrics not been adopted for evaluating GANs.
Inspired by recent work from~\citet{UpchurchGBPSW16} that shows that convolutional neural networks may linearize the pixel-based image manifold, we propose to use the features formed by the last convolutional layer of a third party model pretrained on the ImageNet dataset. For efficiency purposes, we use a 34-layer ResNet\footnote{We used the official pretrained ResNet-34 model from PyTorch \url{http://tinyurl.com/pytorch}.} as the feature extractor. Our experimental results show that other models, e.g., the VGG or Inception networks, lead to very similar outcomes.

%\autoref{fig:robust_shift} shows a simple comparison of distances in the induced space and the original pixel representation.
%We randomly select images from CelebA (see dataset description in \autoref{experiments}), shift them by 4 pixels to the left and find their 10 nearest neighbors in the original dataset. Since the shifted images are semantically identical to the original, we expect a distance metric in a semantically meaningful feature space to include the original as the nearest neighbor.
%As expected, this is realized in the convolutional feature space (right plot), but completely unsuccessful in the pixel and softmax space. A similar observation holds for horizontal flips (see Figure 1 in the appendix).

In the subsequent section, we will show failure examples of using pixel space distance for evaluating GANs, and highlighting that using a proper feature space is a key to obtaining meaningful results when applying any of the distance-based evaluation metrics. The usage of proper feature space enables us to draw more optimistic conclusions on GAN evaluation metrics than \cite{theis2015note} do. In Section \ref{sec:discussion}, we will discuss other possible choices of feature space, such as the convolutional feature space of the VGG or Inception models, random networks or classifiers trained on that specific dataset.

